Reading Comprehension as Natural Language Inference: A Semantic Analysis

In the recent past, Natural language Inference (NLI) has gained significant attention, particularly given its promise for downstream NLP tasks. However, its true impact is limited and has not been well studied. Therefore, in this paper, we explore the utility of NLI for one of the most prominent downstream tasks, viz. Question Answering (QA). We transform the one of the largest available MRC dataset (RACE) to an NLI form, and compare the performances of a state-of-the-art model (RoBERTa) on both these forms. We propose new characterizations of questions, and evaluate the performance of QA and NLI models on these categories. We highlight clear categories for which the model is able to perform better when the data is presented in a coherent entailment form, and a structured question-answer concatenation form, respectively.

==> NLI for QA (StarSem Short Paper for Arxiv)/abstract.tex <==
% Why
In the recent past, Natural language Inference (NLI) has gained significant attention, particularly given its promise for downstream NLP tasks. 
% such as Question Answering and Text Summarization. 
However, its true impact is limited and has not been well studied. 
% What
Therefore, in this paper, we explore the utility of NLI for one of the most prominent downstream tasks, viz. Question Answering (QA).  
% How
% Our analysis focuses on four QA datasets by transforming them into an NLI task. 
We transform the one of the largest available MRC dataset (RACE) to an NLI form, and compare the performances of a state-of-the-art model (RoBERTa) on both these forms. We propose new characterizations of questions, and evaluate the performance of QA and NLI models on these categories.
We highlight clear categories for which the model is able to perform better when the data is presented in a coherent entailment form, and a structured question-answer concatenation form, respectively.

==> NLI for QA (StarSem Short Paper for Arxiv)/appendices.tex <==
% \section{Static passage eval}
%\begin{table*}[!ht]
%\centering
%\begin{tabular}{@{}lllll@{}}
%\toprule
%\multirow{2}{*}{Dataset} & \multicolumn{4}{c}{Dataset Format (conversion method)}          \\ \cmidrule(l){2-5} 
%                         & QA (None) & NLI (Rule-based) & NLI (Neural)      & NLI (Hybrid) \\ \toprule
%RACE                     &   & -                &   &       \\
%RACE-subset              &    &          &            &       \\\midrule
%DREAM                    &    & -                &            &              \\
%DREAM-subset             &           &         &            &       \\\midrule
%MultiRC                  &    & -                &            &       \\
%MultiRC-subset           &    &          &            &      \\\midrule
%BoolQ                    &   & -                &            & -            \\ \bottomrule
%\end{tabular}
%\caption{Accuracy on the dev set with static passage}
%\label{tab:all-results}
%\end{table*}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newpage
\section{Model Architecture}
\label{app:model_arc}
\input{model_arc}

\section{Hyperparameter Settings}
\label{app:hyperparams}
\input{hyperparams}
% \FloatBarrier
\section{Conversion examples}
\label{app:conversion}
\input{conversion_examples}



==> NLI for QA (StarSem Short Paper for Arxiv)/artefacts.tex <==
%As a sanity check, we evaluated both the Rule-based NLI and QA models on an adversarial dev set consisting of examples from the original dev set replaced with static passages of the same length. This test was performed to reveal any artefacts in the data and/or conversion rules that might be resulting in the increase in performance. The results are mentioned in  Table \ref{tab:static-passage-results}. \todo{Fill in Missing Values in the table.}

%Both models gave similar performances, getting about $45\%$ accuracy. While the similar numbers confirm that the gain of the NLI model is not due to artefacts in the conversion rules, the high accuracy achieved by both models is indicative of caveats in the RACE dataset as well as the limitations of RoBERTa as a model.
We first present in Table \ref{tab:static-passage-results}, the performance of the trained models on the \emph{static-passage dev set} as these provide useful information regarding the model performance on the actual dev sets, discussed later.  
For the sake of brevity and easy reference, we call the classification model trained on the input formed by applying the rule-based conversion as the rule-based model.

% \subsection{Evaluation on static-passage dev sets}
For all the datasets in any format, we can see that the evaluation on the static-passage examples produces accuracies higher than random, implying that there are "easy" examples in the dev set which the models can solve without having any useful information in the passage/premise. 

While on RACE and RACE-subset, model trained on any format archives about 42-46\% accuracy on the corresponding static-passage dev set, we observe that on MultiRC the QA models consistently get better accuracy on the static-passage dev set. This indicates that when MultiRC is presented in the QA format, the model finds ways to answer the questions without looking at the passage. On the DREAM dataset, the model achieves about 38\% accuracy in both the QA and NLI formats. This is quite close to random performance, suggesting that the model does in fact use the passage to answer the questions.




%Contrary to the static passage evalutation on RACE-Subset, on the MultiRC dataset the QA version with question and answer concatenation leaks a larger percentage of the answers. As seen from Table \ref{tab:static-passage-results}, the QA model gets $62.2\%$ accuracy on the adversarial MultiRC dev set whereas the NLI model with neural conversions gets only $58.31\%$ which is fairly close to the majority class baseline. \comment{The models do not predict majority class which rules out a naive prediction criterion that the models might have used in the absence of a useful premise. Further, $55\%$ of the accuracy achieved by the QA model overlaps with it's predictions in the static passage setting whereas this overlap is only $44\%$ for the neural NLI model. Thus, the NLI model gains more ($35\%$) than the QA model ($30\%$) when the input contains a relevant premise.} We posit that the model is able to better exploit the artefacts in the dataset when the input is presented in a question-answer concatenation form as opposed to a well formed hypothesis\comment{, however, we are unable to characterize these artefacts}. We use these predictions to divide the dataset into \textit{Hard} and \textit{Easy} and analyse the performance of both the models on the \textit{Hard} questions which neither of the model is able to answer correctly in the static passage setting. The results are discussed in Section \ref{subsec:qualitative_heuristic_cat}.

%We also train the models without the passage/premise, giving only the answer options as input for the RACE-Subset dataset. Figures \ref{fig:random_seed_nli} and \ref{fig:random_seed_qa} show the learning curves of both the models over 3 epochs. Both models achieve close to $50\%$ accuracy with just the answer options further supporting the claim of existence of artefacts in the RACE dataset which the models are able to exploit.

%\begin{figure}[h]
 %   \centering
  %  \includegraphics[width=0.45\textwidth]{images/RandomSeed_NLI.png}
   % \caption{Training Rule-based NLI model without premise. The curves show 10 random seed runs.}
    %\label{fig:random_seed_nli}
%\end{figure}

%\begin{figure}[h]
 %   \centering
  %  \includegraphics[width=0.45\textwidth]{images/RandomSeed_QA.png}
   % \caption{Training QA model without passage. The curves show 10 random seed runs.}
    %\label{fig:random_seed_qa}
%\end{figure}

\begin{table*}[!ht]
\centering
\begin{tabular}{@{}lllllll@{}}
\toprule
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Random} & \multirow{2}{*}{Majority} & \multicolumn{4}{c}{Dataset Format (conversion method)}          \\ \cmidrule(l){4-7} 
                     &&& QA (None) & NLI (Rule-based) & NLI (Neural)      & NLI (Hybrid) \\ \toprule
RACE                    & 25.00 & 26.6 & 42.48& -& 43.01 & 42.95 \\
RACE-subset             & 25.00 & 27.2 & 45.50 & 45.90 & 44.23 & 45.20 \\\midrule
DREAM                   & 33.33 & 34.40 & 37.75 & -& 37.90&38.48\\
DREAM-subset            & 33.33 & 34.20 & 37.04 &37.77 & 38.38 & 38.08 \\\midrule
MultiRC                 & 50.00 & 57.19 & \textbf{62.21} & -& 58.31 & 57.34\\
MultiRC-subset          & 50.00 & 57.46& \textbf{64.19} & 59.6 & 57.80 & 58.00 \\
 \bottomrule
\end{tabular}
\caption{Accuracy numbers on the static-passage dev set with premise replaced with static text of equal length.}
\label{tab:static-passage-results}
\end{table*}


%% DO AGAIN
%Dream-subset QA, DREAM NLI(Neural), RACE-subset NLI(Neural), RACE-subset NLI (Hybrid), RACE NLI (hybrid), MultiRC NLI (hybrid)

==> NLI for QA (StarSem Short Paper for Arxiv)/conclusion.tex <==

There is limited work providing a comprehensive analysis of how NLI can be used for QA.
% \todo{Should we be saying "analysis w.r.t semantics or reasoning"? how about "w.r.t semantic reasoning categories?"}. 
In our work, we show that NLI can be used  for the task of reading comprehension simply by converting the data into NLI form. We convert a large RC dataset into NLI form and perform a comparative study of the performance of the RoBERTa model trained on QA and NLI settings. We propose a categorization of questions that allows for effective comparison of models trained on NLI and QA forms of data. Our analysis clearly shows that using the NLI-based approach is at par with a QA-based approach for most reasoning categories, and it is even better for some. Specifically, we find that questions involving deductive reasoning, dialogue interpretation and math are better handled by a model trained on the NLI form of data than the QA form. However, questions involving negation favor the QA form. Our work allows for careful selection of modeling strategy based on the type of data at hand.
% \lorraine{maybe re-write the conclusion?}
% \kartik{Agreed. The content in here is good, but wrap it around in main claims similar to the abstract/intro. Nicer if you can quantify something.}
% Our experiments also show that the performance of the entailment-based approach is directly affected by the quality of converted data - better the conversion, better the performance. Additionally, we find that there are certain artefacts present in QA datasets which allow the model to answer questions correctly without even reading the given passage.

% Our work lays the grounds for transforming more downstream tasks into an entailment format. If such transformations are successful, NLI could serve as a common abstraction layer for training a model that not only understands the fundamentals of natural language, but is also able to transfer this learned knowledge across different NLP tasks. 


 

   
    
       
%\begin{itemize}
   % \item Solving the task of QA as NLI is as good, if not better
    %\item We show how NLI can be used with the current SoTA models to solve the task of QA
    %\item There are certain categories where NLI does better
    %\item Quality of conversion is important
    %\item We find that major parts of QA datasets can be solved without any useful information from the context
%\end{itemize}

==> NLI for QA (StarSem Short Paper for Arxiv)/contributions.tex <==
\section{Motivation}
\begin{itemize}
    \item 
    NLI is considered a fundamental task in natural language processing. However, application to downstream tasks such as QA is extremely limited with most QA task leaderboards being dominated by complex neural models trained specially for the downstream tasks. NLI-based knowledge transfer models fail miserably when compared to these models. The motivation of our work is to understand the usefulness of NLI and utilize it effectively for Question Answering.

    \item
    The ability to effectively convert downstream NLP tasks to textual entailment would allow the use of a common abstractive layer for training a model that understands the fundamentals of language and is able to transfer this knowledge across NLP tasks.
    
    \item
    State-of-the-art (BERT based) QA models seem to be approaching multiple choice question answering more like an NLI task rather than a QA task. i.e, each answer option is evaluated independently of the others. Restructuring the input and making it even more similar to NLI should boost performance.
\end{itemize}

\section{Contributions}
\begin{itemize}
    \item
    NLI is useful for QA.
    \begin{itemize}
        \item 
        \textit{Qualitative Analysis} of how NLI can be used to enhance QA performance: We present categories of questions which are better solved when posed as an entailment task than a QA task and vice versa.
        \item
        \textit{Quantitative Analysis} of how NLI can be used to enhance QA performance : We show concrete evidence that restructuring input as NLI improves near state-of-the art model performance.
        \item
        Benefits of pre-training and transfer learning ability of the NLI models. [Need to evaluate] 
    \end{itemize}
    
    \item
    BART-based dataset conversion.
    \begin{itemize}
        \item We provide a novel neural based model for effectively converting any QA dataset to NLI format while preserving grammatical structure.
        
        \item Evaluate the conversion on a QA downstream task [Need to evaluate]
        
        \item Better than rule-based conversion [Need to evaluate]
    \end{itemize}
\end{itemize}

\section{Related Work}
\begin{itemize}
    \item 
    No appreciable performance improvements over BERT-like models using NLI. Either prior work does not perform as well as SOTA or doesn't compare to SOTA. \cite{khot2018scitail, clark2018think, Clark, Clark2019, trivedi2019repurposing}

    \item
    Lack of qualitative analysis of NLI and QA tasks to understand model performance. \citet{richardson2019probing} analyse NLI but do not show how these categories might be related to performance on downstream tasks.
    
    \item
    Work done towards converting QA datasets to NLI have largely been rule based and have focused mainly on quality of conversion without attempting to evaluate the conversion on the downstream tasks. \cite{khot2018scitail, clark2018think, Demszky2018, trivedi2019repurposing}
    
    \item
    Pretraining on multiple NLI datasets to improve downstream task performance not done so far.
\end{itemize}


==> NLI for QA (StarSem Short Paper for Arxiv)/conversion_examples.tex <==
%%%%%%%%%%%%%%%%%%% Examples of Conversion %%%%%%%%%%%%%%%%%%%
Table \ref{tab:example_conversions_race} shows examples of NLI-form obtained applying rule-based conversion on QA examples from the RACE-subset.

%%%%%%%%%% RACE %%%%%%%%%%
\begin{table*}[ht!]
    \centering
    \begin{tabular}{p{0.3 \textwidth}|p{0.3\textwidth}}
        \textbf{QA example} & \textbf{NLI-form}  \\ \bottomrule
        \textbf{Q:} How do suburban commuters travel to and from the city in Copenhagen at present?
            \break \textbf{A:} About one third of the suburban commuters travel by bike.
            & Suburban commuters travel to about one third of the suburban commuters travel by bike and from the city in Copenhagen at present.
            \\
        \hline
        \textbf{Q:} What's the best title of the passage?
            \break \textbf{A:} Blame! Blame! Blame!
            & The best title of the passage's blame. 
             \\
        \hline
        \textbf{Q:} What influence did the experiment have on Alexander ?
            \break \textbf{A:} He realized that slowing down his life speed could bring him more content.
            & The experiment had he realized that slowing down his life speed could bring him more content on Alexander.
             \\
        \hline
       \textbf{Q:} Which of the following is TRUE about the report findings?
            \break \textbf{A:} The reading scores among older children have improved.
            & The reading scores among older children have improved is TRUE.
             \\
        \bottomrule
    \end{tabular}
    \caption{Examples of Rule-based  conversion applied to samples from the  RACE-subset. }
    \label{tab:example_conversions_race}
\end{table*}



==> NLI for QA (StarSem Short Paper for Arxiv)/converting_QA2NLI.tex <==

%\kartik{Consider re-organizing this section to talk first about the conversion of QA to NLI, and the models being used. Then you can bring in the dataset part. It should also be called something other than ``experimental setup'', which makes the transition from related work seem very abrupt.}

We use the RACE dataset \cite{lai2017race} for our experiments. It is a large-scale reading comprehension dataset comprising of questions collected from the English exams for junior Chinese students. Each question contains four answer options, out of which only one is correct. %(see Figure \ref{fig:conversion}a). 
However, about 44\% of the RACE dataset consists of cloze style (fill-in-the-blank) questions which are already in NLI form. Hence, in order to have a fair comparison, we only use the subset of RACE dataset which does not contain cloze style questions. This subset consists of $48890$ train, $2496$ validation and $2571$ test examples.


We convert a RC example into an NLI example by reusing the passage as premise and paraphrasing the question along with each answer option as individual hypotheses as shown in Figure \ref{fig:conversion}. Specifically, we generate the dependency parse of both the question and the answer option by using Stanford NLP package \cite{stanfordnlp}, then we follow the conversion rules proposed in \citet{Demszky2018} to generate a hypothesis sentence\footnote{Appendix \ref{app:conversion} presents example conversions generated using these rules.}. We make a few additions to these rules to handle a some peculiar question categories in the RACE dataset. The most prominent of the added rules is the one for questions containing \textit{``which of the following are (not) true''}. Such questions are very frequent (about 6\% of all questions) and are not handled correctly by the rules in \citet{Demszky2018}. 
 



==> NLI for QA (StarSem Short Paper for Arxiv)/entailment_examples.tex <==
% \begin{table*}[!ht]
%     \centering
%     \begin{tabular}{p{3.5cm}|p{5.5cm}|p{5.5cm}}
%         \toprule
%         \textbf{Premise} & A senior is waiting at the window of a restaurant that serves sandwiches & \textbf{Relationship}\\
%         \bottomrule
%         \multirow{3}{*}{\textbf{Hypothesis}}& A person waits to be served his food & Entailment  \\
%         & A man is looking to order a grilled cheese sandwich & Neutral  \\
%     & A man is waiting in line for the bus & Contradiction \\
%         \bottomrule
%     \end{tabular}
%     \caption{Example of Natural Language Inference}
%     \label{tab:nli_example}
% \end{table*}

\begin{table*}[!ht]
    \centering
    \begin{tabular}{p{0.3\textwidth}|p{0.6\textwidth}}
        \toprule
        \textbf{Premise} & \textbf{Hypothesis}\\
        \bottomrule
        \begin{flushleft}
        A senior is waiting at the window of a restaurant that serves sandwiches\end{flushleft}
        & \begin{flushleft} (Entails)\break\textbf{Entailment:} A person waits to be served his food. \break
        
        (Not Entails)\break
        \textbf{Neutral:} A man is looking to order a grilled cheese sandwich. \break
        \textbf{Contradiction:} A man is waiting in line for the bus. \end{flushleft}\\
        \bottomrule
    \end{tabular}
    \caption{Example of Natural Language Inference}
    \label{tab:nli_example}
\end{table*}

==> NLI for QA (StarSem Short Paper for Arxiv)/experiments.tex <==
\subsection{Datasets}
\label{sec:datasets}
%\guide{Please list which datasets you plan to use , whether or not you have access them, and whether or not they are publicly available with the same preprocessing and train / dev / tests as the previous work you will be comparing to (if applicable).}
%\points{Write why we picked RACE. Problems with ARC/SciTail. What are the other datasets which we might use to establish/generalize our findings. How we are converting RACE dataset. }

While there are several QA datasets available, we will use RACE \cite{lai2017race}, MultiRC \cite{multirc} and OpenBookQA \cite{openbookqa} for our analysis, as these datasets provide variety in terms of the types of reasoning required to answer a question while also giving us an opportunity to compare our findings to other related work \cite{Trivedi2019}. 


The analysis in this work is focused on the task of multiple choice question answering. In order to compare the performance of the system using a QA model to that of the one using an NLI model, we will convert the QA datasets to NLI format where the question and answer option will be used to create a hypothesis sentence while the premise will consist of the passage/context text as shown in the figure \ref{fig:conversion_nli}. In order to perform the conversion, we will first employ rule based methods from \cite{Trivedi2019,Demszky2018} and move on to a neural conversion model proposed in \cite{Demszky2018} should we find the quality of rule based conversion unsatisfactory. 

 \begin{figure*}[!h]
    \centering
    \includegraphics[width=\linewidth]{images/conversion_pure_nli.png}
    \caption{Conversion of a QA sample into four NLI samples to be used in ``pure NLI'' setting.}
    \label{fig:conversion_nli}
\end{figure*} 

\subsection{Models}
%\guide{Please list the baseline methods (if applicable) that you will compare to, importantly state whether or not you will need to run their method on new datasets or if you have already published results. Also list if they have publicly available source code that can be used to run experiments.}



We divide our models into two general categories, namely large scale language model based (LSLM) and small entailment models (SEM). The LSLM category consists of RoBERTa \cite{liu2019roberta} and BERT \cite{devlin2018bert} sentence classification models consisting of the corresponding pretrained masked language model encoder at the base with sequence classification head. While SEM models consist of decomposable attention model (DecompAttn) \cite{parikh2016decomposable} and enhanced LSTM for NLI (ESIM) \cite{Chen} which are trained from scratch. Including these two categories of models in our analysis will help us quantify the effect of large scale pretraining with masked language modelling objective on the task of question answering through natural language inference.


\subsection{Training and Evaluation}
\label{sec:training}
We conduct experiments using two strategies. In one, which we call ``NLI with options'', we train and evaluate the model in a QA-like setting where each sample is treated as a 4-way classification problem as shown in the figure \ref{fig:conversion_nli_with_options} (right). The hypotheses for all of the answer options are fed to the network along with the premise (passage) to obtain a joint distribution over the hypothesis options. The only difference between this and a QA setting is that instead of feeding the model four question-option pairs we give the model four hypothesis statements from which it has to choose the most suitable one. This setting allows us to isolate the effect of presenting the options as well-formed hypothesis sentences instead of question+option sequence.

Alternatively, we also train and evaluate models in a much harder ``pure NLI'' setting where the hypothesis corresponding to each answer option is treated as an individual example during training. At evaluation time, we use the NLI scores - which are the scores obtained by passing each premise-hypothesis pair to the NLI model and select the correct answer as the option that gets the best score. This harder training objective forces the model to look for more evidence while selecting an answer hypothesis and is also suited for QA datasets like MultiRC where multiple options can be correct simultaneously.

\begin{figure*}[!h]
    \centering
    \includegraphics[width=\linewidth]{images/conversion_nli_with_options.png}
    \caption{Conversion of a QA sample into a single NLI sample to be used in the ``NLI with options'' setting.}
    \label{fig:conversion_nli_with_options}
\end{figure*} 
%\points{Two categories of models: LM based and non-LM based models. }

\subsection{Updates since the project proposal presentations}
%\points{Put the analysis from the dropbox paper}

We converted the RACE dataset into an entailment-based QA dataset as described in section \ref{sec:datasets}. We trained RoBERTa sequence classification model in both settings ``pure NLI'' as well as ``NLI with options'' and compared its performance to a RoBERTa QA model (trained on RACE dataset as it is). The accuracy on the dev dataset for all three settings is similar.
%shown in the table \ref{tab:roberta}. \lorraine{where is the table?}


%\begin{table*}[!ht]
%\centering
%\begin{tabular}{@{}llll@{}}
%\toprule
%Model   & \multicolumn{3}{c}{Accuracy on QA dev set} %              \\ \midrule
%        & Trained as QA & Trained as Pure NLI & Trained as NLI with options \\ \midrule
%RoBERTa-large &               &                     &                             \\ \bottomrule
%\end{tabular}
%\caption{Results for RoBERTa-large}
%\label{tab:roberta}
%\end{table*}


Even though the models perform similarly in all three settings, a deeper error analysis provides some interesting observations. While the RoBERTa QA model performs well on questions which can be answered using the surface information and which do not require multi-hop or complex reasoning, it fails to answer questions which require deeper understanding of the passage -- questions asking about a suitable title for the passage, or ones which ask about intentions of the author or people mentioned in the passage.


 
\subsection{Software}
We are using various set of open-source libraries for different subparts of this work. 
\begin{itemize}
    \item \textbf{Models}: While we are using HuggingFace's transformer\footnote{https://github.com/huggingface/transformers} library \cite{Wolf2019HuggingFacesTS} for pretrained language models like RoBERTa and BERT, we are using AI2's AllenNLP\footnote{https://github.com/allenai/allennlp/} \cite{Gardner2017AllenNLP} library to implement models like ESIM and DecompAttn. 
    
    \item \textbf{Analysis and Labeling}: We are using Label Studio \footnote{https://github.com/heartexlabs/label-studio} -- a multi-type data labeling and annotation tool -- for analysing, labelling and categorizing of our data.
    
    \item \textbf{Training management and hyperparameter tuning}: We are using Weights \& Biases\footnote{https://www.wandb.com/} \cite{wandb} to manage our experiments.
\end{itemize}



\subsection{Timeline}
%\guide{Please provide a week-by-week timeline for the next few weeks leading up to the midpoint presentations. What experiments will you do each week? What would you like to have accomplished by the midterm? If you're in a team how will you divide up the work?}

\begin{itemize}
    \item 03/08 - 03/14: 
    \begin{itemize}
        \item Implement ESIM and DecompAttn and train under all three settings mentioned in \ref{sec:training} (Dhruvesh)
        \item Implement other models in the LSLM category and train under all three settings (Anshuman)
        \item Categorize the erroneous as well correct predictions from RoBERTa sequence classification model on RACE as ``pure NLI'' and ``NLI with options'' and compare it with the errors made by the RoBERTa QA model on the RACE dataset (Aparna)
    \end{itemize}
    \item 03/15 - 03/21:
    \begin{itemize}
        \item Evaluate all the models on MultiRC and OpenBookQA in all three training settings (Dhruvesh, Anshuman, Aparna)
    \end{itemize}
    \item 03/21 - 03/27:
    \begin{itemize}
        \item Perform error analysis for all the models on all the datasets. Come up with general observations based on model category and dataset (Dhruvesh, Anshuman, Aparna)
        \item Work on mid-point presentation (Dhruvesh, Anshuman, Aparna)
    \end{itemize}
\end{itemize}

\subsection{Challenges}
%\guide{Lay down the challenges that you can foresee which might prevent you from attaining your goal.}

We are already facing several challenges and following are the major ones.

\begin{enumerate}
    \item \textbf{Grammaticality of hypothesis}: Due to the richness and variety of the questions, rule based methods to convert a question+answer option to a hypothesis sentence, in some cases, produce grammatically incorrect sentences. Currently, for the converted RACE dataset, we have identified that about 20\% of the total hypothesis sentences are grammatically incorrect. As this is a significant fraction, we continue to improve the employed rules to convert all such examples correctly. Since this aspect is not the  focus of this work, we do not wish to spend a lot of time on improving the conversion strategy.
    
    %\lorraine{how much percent of the converted sentence is un-grammatical? If not too much, we don't have to worry about this. But if it's a lot, maybe we should see the performance difference if we manually change some of the sentence into grammatically correct one?}
    
    \item \textbf{Long premise length}: Since the passage/context directly acts as the premise, on an average, we deal with premise sequences of 300 or more tokens. This poses two challenges. One, we cannot directly employ some of the BiLSTM based NLI models like ESIM as they cannot handle such long premise directly. Secondly, we cannot transfer learn from existing NLI datasets. We address the first issue by using Multee \cite{Trivedi2019} which employs small entailment models like ESIM with importance weighting and aggregation. 
\end{enumerate}


%\subsection{Contingency Plan}


==> NLI for QA (StarSem Short Paper for Arxiv)/further_exp.tex <==
\begin{itemize}
    \item
    Evaluate model performance with neural converted dataset.
    
    \item 
    Evaluate other datasets
    \begin{itemize}
        \item \textit{DREAM} - a multiple-choice Dialogue-based REAding comprehension exaMination dataset. \cite{sun2019dream} 
        
        It contains 10,197 multiple choice questions for 6,444 dialogues, collected from English-as-a-foreign-language examinations designed by human experts. 
        
        The dataset is likely to present significant challenges for existing reading comprehension systems: 84\% of answers are non-extractive, 85\% of questions require reasoning beyond a single sentence, and 34\% of questions also involve commonsense knowledge. 
        
        \item \textit{MultiRC} - a dataset of short paragraphs and multi-sentence questions that can be answered from the content of the paragraph. \cite{MultiRC2018}
        
        The entire corpus consists of ~10K questionss (~6k multiple-sentence questions). We release about 60\% of this data as training/dev data.
 
    \end{itemize}
    
    \item 
    Refine categories and perform more annotation.
    
    \item 
    Pre-train on other NLI datasets and evaluate performance.
\end{itemize}

==> NLI for QA (StarSem Short Paper for Arxiv)/hyperparams.tex <==
%\vspace{-100mm}
\begin{table}[!ht]
    \centering
    \begin{tabular}{l|c c}
        \multirow{2}{*}{\textbf{Hyperparam}} 
        & \multicolumn{2}{c}{\textbf{RACE-subset}} \\
        & \textbf{NLI-form} & \textbf{QA-form}  \\
        \bottomrule
        learning rate & 1e-5 & 1e-5  \\ \hline
        weight decay & 0.01 & 0.01 \\ \hline
        warmup steps & 1300 & 1300 \\ \hline
        batch size & 16 & 16 \\ \hline
        max epochs & 4 & 4 \\
        \bottomrule
    \end{tabular}
    \caption{Hyperparamter Setting}
    \label{tab:hyperparams}
\end{table}

Table \ref{tab:hyperparams} lists the hyperparameter settings for both versions of the dataset.

==> NLI for QA (StarSem Short Paper for Arxiv)/intro_3.tex <==
% Why NLI?
%Natural Language Inference (NLI) has always been considered a critical task for Natural Language Understanding~\cite{wang2018glue}. 
Given two sentences, a premise and a hypothesis, the task of Natural Language Inference (NLI) is to determine whether the premise entails the hypothesis or not. \footnote[2]{The ``not entailment'' can further be subdivided into ``neutral'' and ``contradiction''. However, we only use the two-class version of the problem in this work.} 
%An example of NLI taken from the Stanford Natural Language Inference Corpus \cite{Bowman2015} is shown in Table~\ref{tab:nli_example}.
%Recent works in NLI have focused on assembling larger and more diverse datasets~\cite{Bowman2015,williams2017broad,khot2018scitail,Guo2018} which has led to better and more sophisticated models for NLI. Most of these popular NLI datasets appear to be solved with state of the art models achieving very close to human performance.
%\input{entailment_examples}
%%%% So NLI is cool, and we seem to have aced it, but how can we really use it? Have we been able to use it for downstream tasks?
The concept of semantic entailment is central to natural language understanding \cite{van2008brief, maccartney2009natural} and therefore,  NLI models have been used to help with various downstream tasks like reading comprehension \cite{Trivedi2019},  summarization \cite{falke2019ranking,kryscinski2019evaluating}, and dialog systems \cite{dnli}. However, the performance of an NLI system on these downstream tasks has not been studied with respect to semantic or reasoning categories.
%\lorraine{However, the transfer of the semantics contained in the NLI-formatted task to the downstream task have not been clearly studied.}
%It also gives rise to the hope of forming a common layer of reasoning which can efficiently transfer language knowledge across inherently different downstream tasks. However, efforts towards transferring the knowledge of state-of-the-art NLI models for downstream tasks has had limited success so far ~\cite{clark2018think, falke2019ranking, Trivedi2019}.

In this work, we use NLI to perform the task of multiple choice reading comprehension (MRC, or RC). We analyse the performance of an NLI model on this task through the lens of semantics by identifying the reasoning categories (type of questions) where it is beneficial to use an NLI model.

% Do we know why? What have people tried? What can we do?
%We opt for QA as an end task for the following reasons: (1) QA is a popular task for Natural Language Understanding with diverse datasets that can be leveraged for our analysis. (2) Intuitively, it is easy to see that QA naturally reduces to an two-class NLI problem \todo{refer to the example here}, specifically, identifying if some text entails the answer to a question or not. 

% SciTail \cite{khot2018scitail} is a manually curated science-focused NLI dataset designed as a parallel dataset to the science-focused QA dataset - ARC \cite{clark2018think}. It is natural to expect in-domain models to be better at knowledge transfer, however, pre-training on SciTail fails miserably on ARC, barely being able to break the random baseline. \citet{Demszky2018} train a neural model to show a generalized way of converting any QA dataset to an NLI form. However, they do not discuss the utility of the converted dataset on any downstream task. \citet{Trivedi2019} attribute the difficulty in transferring knowledge to long passages in QA tasks. They show that it's possible to repurpose pre-trained NLI models for question answering by combining sentence level entailment representations. Their model however, considerably underperforms when compared to the state-of-the-art models. 

%Several prior works have attempted to blend NLI into the task of QA with minimal success \cite{khot2018scitail, clark2018think, Demszky2018, Trivedi2019}.
%While there have been hints of NLI being useful, there is little qualitative understanding of when it might be useful. In our work, we aim to perform a thorough analysis to understand the types of problems more suited to NLI and QA forms respectively. 

% \citet{Clark2019} show that pre-training on NLI datasets boosts model performance on naturally occurring yes/no questions. In our work, we highlight that merely converting the dataset to a coherent entailment form can achieve similar improvements in performance.

% So what are we doing different?
% Recent research has highlighted various caveats in the popular large-scale NLI datasets \cite{Gururangan2018, Geva2019, Ravichander2019}, making pre-training and transfer of knowledge a difficult proposition. We argue that present state-of-the-art models such as RoBERTa \cite{liu2019roberta} already view the task of QA as entailment with the concatenation of question and individual answer options; along with the passage posed as a 2 sequence classification task to the model. It is therefore intuitive to believe that forming grammatically coherent hypotheses would lead to improvement in model performance. Further, being able to effectively convert datasets to an entailment form would help overcome the bottleneck of having well structured NLI datasets for pre-training. 

Drawing inspiration from the prior work in the area \cite{clark2018think, Demszky2018, Trivedi2019}, we use rule-based conversion to create an NLI version of the largest available RC dataset - RACE \cite{lai2017race}. We train a RoBERTa based RC model on the original dataset, and a similar RoBERTa based NLI model on the NLI version of the dataset. We evaluate and analyse the performance of both these models by characterizing the question types that are better suited for an NLI model and a QA model.

==> NLI for QA (StarSem Short Paper for Arxiv)/model.tex <==


In order to perform apple-to-apple comparison we use the same model architecture for both QA and NLI. Specifically, we use the state-of-the-art reading comprehension model -- consisting of a RoBERTa model (pretrained on the masked language modeling objective) as the encoder and a two layer feed-forward network on its [CLS] token as the classification head -- as described in \citet{liu2019roberta}. The input sentence is the combination of the passage and its hypothesis. The hypothesis are created using the rule-based conversion method mentioned in Section \ref{sec:conversion} (NLI setup) or by concatenation of question and answer option (QA setup). 


==> NLI for QA (StarSem Short Paper for Arxiv)/model_arc.tex <==


Figures \ref{fig:model_qa} and \ref{fig:model_nli} show the model architecture for the QA and NLI models, respectively. As seen the architecture of the model is the same, the only difference is in the input form.
\begin{figure*}
    \centering
    \includegraphics[width=0.7\textwidth]{images/RoBERTa_qa.png}
    \caption{QA model}
    \label{fig:model_qa}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.7\textwidth]{images/RoBERTa_NLI.png}
    \caption{NLI model}
    \label{fig:model_nli}
\end{figure*}



==> NLI for QA (StarSem Short Paper for Arxiv)/qualitative_analysis.tex <==







%\subsubsection{Manual analysis}
In order to perform manual analysis, we construct a \emph{delta subset} consisting the $328$ dev set examples on which the predictions of the QA and NLI models differ.
We further divide the \emph{delta subset} into \emph{gain} and \emph{loss} subsets. The \emph{gain subset} consists of questions which the NLI model gets right, but the QA model gets wrong, and the \emph{loss subset} is its complement in the \emph{delta}. 

\begin{table*}[!ht]
\begin{tabular}{p{1.8cm}|p{5.2cm}|p{8.6cm}}
\toprule
\textbf{Category} & \textbf{Description} & \textbf{Example} \\ \midrule
Linguistic Matching & Matching words between the question and a sentence in the passage & \textbf{Passage} : Food cooks quickly in parabolic cookers \\
 &  & \textbf{Question}: If you want to cook food quickly, which kind of sun-cooker is your best choice? \\ \midrule
Main Idea & Require topicality judgements & What's the best title for this passage? \\ \midrule
Negation & Picking the incorrect statement & Which of the following statements is NOT true? \\ \midrule
Dialogue & Can be inferred from a dialogue or direct speech in the passage & By saying "her pen dared travel where her eyes would not", the writer means \\ \midrule
Math & Mathematically combining facts & How many functions of snow are discussed in the text? \\ \midrule
Deductive & None of the above but can be answered precisely from the text & Which of the following statements is TRUE? \\ \midrule
Inductive & None of the above and cannot be answered precisely from the text & How old is most likely the writer's father? \\ \bottomrule
\end{tabular}
\caption{Reasoning Categories (exclusive)}
\label{tab:reasoning_categories}
\end{table*}

We manually annotate these $328$ ($192$ in \emph{gain} and $136$ in \emph{loss}) examples into one of the $7$ categories. However, about half the examples in the \emph{delta subset} were not properly converted by the rules leading to unnatural or incoherent hypothesis sentences. Hence, for the purpose of illustration, we removed these examples leaving a total of $175$ examples ($109$ in \emph{gain} and $66$ in \emph{loss}) to do further analysis. Figures \ref{fig:gain_dist} and \ref{fig:loss_dist} show the distribution of labels over the Gain and Loss regions respectively. The distribution reflects that the QA models clearly outperforms the NLI model in negation questions whereas the NLI model outperforms the QA model in dialogue and deductive reasoning categories.

\begin{table*}[]
    \centering
    \begin{tabular}{p{0.15\textwidth}|p{0.85\textwidth}}
        \toprule
        \textbf{Type} & \textbf{Heuristics} \\
        \bottomrule
        Main Idea & Questions containing the words 'mainly', 'title', 'purpose' or 'topic'\\\hline
        Negation & Questions containing the 'not', 'except' or 'which of the following is wrong'\\\hline
        Dialogue & Passages containing more than 10 quotation marks (")\\\hline
        Math & Questions containing the words 'how many', 'how old' or 'how much'\\\hline
        Deductive & Questions containing the word 'true'\\%\hline
        %Fill in the Blanks (FITB) & Questions containing a blank (\_)\\
        \bottomrule
    \end{tabular}
    \caption{Heuristically Determined Question Types in RACE-subset (non-exclusive).}
    \label{tab:heuristic_categories}
\end{table*}

\begin{figure}[!ht]
% \hspace{-15mm}
\includegraphics[width=0.45\textwidth]{images/Gain_QAvsRule_largerfont.png}
\caption{Reasoning categories of the gain region}
\label{fig:gain_dist}
\end{figure}

\begin{figure}[!ht]
    % \hspace{-15mm}
    \includegraphics[width=0.45\textwidth]{images/Loss_QAvsRule_largerfont.png}
    \caption{Reasoning categories of the loss region}
    \label{fig:loss_dist}
\end{figure}

\subsection{Categories based on heuristics}
We also define another set of non-exclusive categories using heuristics, as described in Table \ref{tab:heuristic_categories}. 
 As shown in Table \ref{tab:heuristic_categories_perf}, the NLI model outperforms the QA model significantly in the dialogue, math and deductive reasoning categories. 
 This overall trend further emphasizes the benefits of proper hypothesis generation as opposed to question and answer concatenation for the reading comprehension task.



\begin{table}[]
    \centering
    \begin{tabular}{c|c|c|c}
        \toprule
        \textbf{Type} & \textbf{Fraction} & \textbf{QA} & \textbf{NLI} \\
        \bottomrule
        Main Idea & 0.12 & 84.19 & 84.83\\\hline
        Negation & 0.06 & \textbf{80.86} & 77.77 \\\hline
        Dialogue & 0.12 & 80.65 & \textbf{83.60} \\\hline
        Math & 0.03 & 45.00 & \textbf{55.00} \\\hline
        Deductive & 0.04 & 81.91 & \textbf{88.29} \\%\hline
        %FITB & 0.11 & 79.02 & 79.02 \\
        \bottomrule
    \end{tabular}
    \caption{Model performances on heuristically determined question types for RACE-Subset.}
    \label{tab:heuristic_categories_perf}
\end{table}



==> NLI for QA (StarSem Short Paper for Arxiv)/quantitative_analysis.tex <==
\begin{table}[]
\centering
\begin{tabular}{@{}lllll@{}}
\toprule
\multirow{2}{*}{Dataset} & \multicolumn{2}{c}{Dataset Format}          \\ \cmidrule(l){2-3} 
                         & QA & NLI \\ \toprule
RACE                     & \textbf{85.78}  & -                   \\
RACE-subset              & 79.84   & \textbf{82.09}       \\\bottomrule
\end{tabular}
\caption{Accuracy on the test set obtained by using different formats of the data.}
\label{tab:all-results}
\end{table}

%\todo{This acc is on dev set because we perform analysis on dev set. Is this bad? It's fine to do analysis dev set, but I think we should report test set accuracy as well. Can we get those easily?}

Table \ref{tab:all-results} shows the accuracy achieved by the RoBERTa model on the RACE dataset and its subset when presented in different forms. \label{subsec:quantitative_race} As we can see, the NLI model performs much better than the QA model on RACE subset.
% We believe that the reason for this could be the more natural form of the hypothesis statement used by the NLI model compared to the Q+A concatenation from used by the QA model. The model sees sentences in their natural form rather than Q+A form during its pre-training with masked language modeling objective.
We think that the reason for this is the more natural form of the hypothesis statement used by the NLI model compared to the Q+A concatenation form used by the QA model.
Moreover, while the RACE-subset consists of only those questions which have question-words such as \{\textit{who, what, when...}\}, about $95\%$ of the rest of the dataset, i.e. RACE $\setminus$ RACE-subset, consists of only fill-in-the-blank (FITB) type questions. These FITB questions are largely with the blank at the end of the question and a naive question-answer concatenation is very similar to a NLI form hypothesis. We believe that helps the QA model to perform better on the full RACE dataset compared to the RACE-subset, where NLI model is able to outperform the QA model showing the clear benefits of coherent conversion on complex question formulations (such as \textit{W} word questions).

In order to analyse the performance difference from a semantic perspective, we characterize question into $7$ semantic categories by identifying the kind of reasoning required to answer the question. Table \ref{tab:reasoning_categories} succinctly describes the reasoning categories. 



==> NLI for QA (StarSem Short Paper for Arxiv)/reasoning_categories.tex <==
In order to get a qualitative understanding of the differences between the two settings, we divide the questions into $7$ categories reflecting the type of reasoning required to answer the question. Table \ref{tab:reasoning_categories} describes these reasoning categories along with examples.

\begin{table*}[!ht]
    \centering
    \begin{tabular}{p{3.5cm}|p{5.5cm}|p{5.5cm}}
        \toprule
        \textbf{Category} & \textbf{Description} & \textbf{Example}\\
        \bottomrule
        Linguistic Matching & Can be answered merely by matching words between the question and a sentence from the passage & \textbf{Passage Sentence:} Food cooks quickly in parabolic cookers \\ & & \textbf{Question:}If you want to cook food quickly, which kind of sun-cooker is your best choice?\\\hline
        Main Idea & Require topicality judgements & What's the best title for this passage?\\\hline
        Negation & Picking the wrong/incorrect statement & Which of the following statements is NOT true?\\\hline
        Dialogue & Can be inferred from a dialogue or direct speech in the passage & By saying "her pen dared travel where her eyes would not", the writer means\\\hline
        Math & Counting or mathematically combining facts & How many functions of snow are discussed in the passage?\\\hline
        Deductive & None of the above but can be answered precisely from the premise text & Which of the following statements is TRUE?\\\hline
        Inductive & None of the above and cannot be answered precisely from the text & How old is most likely the writer's father?\\
        \bottomrule
    \end{tabular}
    \caption{Reasoning Categories}
    \label{tab:reasoning_categories}
\end{table*}

We construct the delta region as the $328$ dev set examples on which the predictions of the QA and Rule-based NLI models differ. We further divide the Delta region into Gain (NLI gets it right, QA gets it wrong) and Loss (QA gets it right, NLI gets it wrong). We annotate these $328$ ($192$ in Gain and $136$ in Loss) examples into one of the $7$ categories. The annotation process also revealed that about half the examples were not properly converted by the rules leading to grammatical errors or loss of information in conversion. For the purpose of our analysis, we removed these examples leaving a total of $175$ examples ($109$ in Gain and $66$ in Loss). However, it's worth noting that the presence of bad conversions affects the scope of learning of the model in addition to the fact the fraction of incorrect conversions was higher in the Loss region. These observations suggest that improving upon conversion could further boost performance.

Figure \ref{fig:gain_dist} and \ref{fig:loss_dist} show the distribution of labels over the Gain and Loss regions respectively. The distribution reflects that the QA models clearly outperforms the NLI model in negation questions whereas the NLI model outperforms the QA model in dialogue and deductive reasoning categories.

\begin{figure}[h]
\includegraphics[width=0.45\textwidth]{images/Gain_QAvsRule.png}
\caption{Distribution of Reasoning Categories over the Gain region - Rule-based NLI vs QA model}
\label{fig:gain_dist}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{images/Loss_QAvsRule.png}
    \caption{Distribution of Reasoning Categories over the Loss region - Rule-based NLI vs QA model.}
    \label{fig:loss_dist}
\end{figure}

==> NLI for QA (StarSem Short Paper for Arxiv)/reasoning_categories_heuristical.tex <==
\begin{table*}[!ht]
    \centering
    \begin{tabular}{p{0.25\textwidth}|p{0.65\textwidth}}
        \toprule
        \textbf{Type} & \textbf{Heuristics} \\
        \bottomrule
        Main Idea & Questions containing the words 'mainly', 'title', 'purpose' or 'topic'\\\hline
        Negation & Questions containing the 'not', 'except' or 'which of the following is wrong'\\\hline
        Dialogue & Passages containing more than 10 quotation marks (")\\\hline
        Math & Questions containing the words 'how many', 'how old' or 'how much'\\\hline
        Deductive & Questions containing the word 'true'\\\hline
        Fill in the Blanks (FITB) & Questions containing a blank (\_)\\
        \bottomrule
    \end{tabular}
    \caption{Heuristically Determined Question Types - RACE}
    \label{tab:heuristic_categories}
\end{table*}

As a consequence of the rule-based conversion strategy, we unintentionally get 2 very different sets of data from the RACE dataset. $83\%$ of the RACE-subset consists of questions with question-words such as \{\textit{who, what, when, where, why, which, how}\} whereas only $1\%$ of the rest of the RACE dataset has such questions. Conversely, only about $11\%$ of the subset consists of fill-in-the-blanks (FITB) questions whereas $95\%$ of the rest of the dataset has FITB questions. \comment{FITB questions are largely with the blank towards the end of the question and a question-answer concatenation strategy turns out to be very similar to a coherent conversion strategy. We argue that this is the reason for equivalent performance of the models on the FITB part of the data. However, on the RACE-subset, NLI models are able to outperform the QA model which showing the clear benefits of coherent conversion on complex question formulations.}

In order to compare the models trained using the neural and hybrid conversion to the rule-based conversion, we define some non-exclusive categories using heuristics, as described in Table \ref{tab:heuristic_categories}. We observe that the NLI model which uses the hybrid conversion gets a significantly better performance on the deductive reasoning category than the NLI model which uses the rule-based conversion. This observation is consistent with the trend seen in the comparison of the rule-based model vs the QA model, where the rule-based model outperforms the QA model on the deductive reasoning category. Additionally, the rule-based model outperforms the QA model significantly in the dialogue category. Table \ref{tab:heuristic_categories_perf} shows the performance of the models on the RACE-subset dataset over these question types. This trend further emphasizes the benefits of proper hypothesis generation as opposed to question and answer concatenation for the question-answering task.

On the Multi-RC dataset, we created question types by following heuristics similar to those used in the orignal paper to analyse the dataset distribution. The question types and their proportion in the dataset is described in Table \ref{tab:heuritic_categories_multirc}. We analyse the performance of both the QA and neural-conversion NLI model across these categories. Specifically, we analyse the changes in trend on the subset of \textit{Hard} questions (Section \ref{subsec:qualitative_artefacts}). The distribution across categories does not change in the restricted set of \textit{Hard} questions which indicates that the artefacts are not specific to any of these question types. We observe that the NLI model outperforms the QA model on \textit{assertion} and \textit{when} types and matches QA performance on \textit{how} questions. To further understand the performance gap, we looked examples from these different categories and found that there are certain complexities in the questions which neural conversion is unable to handle. These include questions with multiple answers, examples where the answer is also a question and examples with partially correct answers labelled as true in the dataset. Table \ref{tab:multirc_hard_examples} provides some examples of these. Such examples are also a major cause for incorrect conversions. It is particularly interesting to note that such difficult examples are present in \textit{what} and \textit{who} in large proportions and almost completely absent from question types such as \textit{assertion}. This could be the primary reason for the inability of the NLI model to beat or even match QA model performance on these categories. We conclude that MultiRC is a harder dataset for NLI in the constraints of the rules and neural model we have trained. The dataset has nuances which need to be captured during conversion to be able to outperform the QA model.

\begin{table}[!ht]
    \centering
    \begin{tabular}{c|c|c|c}
        \toprule
        \textbf{Type} & \textbf{QA} & \textbf{Rule-based} & \textbf{Hybrid}\\
        \bottomrule
        Main Idea & 84.19 & \textbf{84.83} & \textbf{84.83}\\\hline
        Negation & \textbf{80.86} & 77.77 & 79.01\\\hline
        Dialogue & 80.65 & \textbf{83.60} & 82.95\\\hline
        Math & 45 & \textbf{55} & \textbf{55}\\\hline
        Deductive & 81.91 & \textbf{88.29} & \textbf{90.42}\\\hline
        FITB & 79.02 & 79.02 & \textbf{79.40}\\
        \bottomrule
    \end{tabular}
    \caption{Model performances on heuristically determined question types for RACE-Subset}
    \label{tab:heuristic_categories_perf}
\end{table}


\begin{table*}[!ht]
    \centering
    \begin{tabular}{@{}l|p{0.35\textwidth}|p{0.35\textwidth}@{}}
    \toprule
        \textbf{Type} & \textbf{Heuristic} & \textbf{Example}\\
    \toprule
        what (40\%) 
 & Starts With ['What', 'In what', 'With what', 'To what'] or Ends With [‘what?’]
 & What is the drawback of kinetic energy from hydro power? \\ \hline
        who (15\%) & Starts With ['Who', 'Whom', 'With whom', 'From whom', 'For whom'] or Ends With [‘who?’, ‘whom?’] & Who does Billy have the same color hair as?\\ \hline
        how (12\%)& Starts With [‘How’] & Approximately how much older is Charlie than Sylvia?\\ \hline
        why (10\%)& Starts With [‘Why’] & Why did Phoebe cry?\\ \hline
        assertion (5\%)& Starts With ['Could it', 'Will ', 'Was', 'Were', 'Has', 'Have', 'Does', 'Would', 'Did', 'Had', 'Is', 'Are', 'Do', 'Can', 'True or false'] & Was the Emperor hurt when the explosion damaged his carriage?\\ \hline
        which (5\%) & Starts With ['Which', 'In which'] & Which philosopher is said to have taught the young Confucius?\\ \hline
        double questions (4.5\%) & Contains ['and what', 'and how', 'and which', 'and where', 'and when', 'and why', 'and by whom', 'if not, what?'] or count("?") $>$ 1 & Where did money to fund the 9/11 plotters come from and where didn't it come from?\\ \hline
        when (3\%) & Starts With [‘When’]
 & When did the Romans set up a fortress at Aquae Sextiae (Aix-en-Provence)?\\ \hline
        where (3\%) & Starts With [‘Where’] or Ends With [‘where?’]
 & Where does the absorption part of digestion occur?\\
    \bottomrule
    \end{tabular}
    \caption{Heuristicaly Determined Question Types - MultiRC}
    \label{tab:heuritic_categories_multirc}
\end{table*}

\begin{table*}[!ht]
    \centering
    \begin{tabular}{@{}lcccc@{}}
    \toprule
        \multirow{2}{*}{\textbf{Type}} 
            & \multicolumn{2}{c}{\textbf{All Questions}} & \multicolumn{2}{c}{\textbf{Hard Questions}}\\
            \cmidrule(l){2-3} \cmidrule(l){4-5} 
            & \textbf{QA} & \textbf{NLI (Neural)} & \textbf{QA} & \textbf{NLI (Neural)} \\
    \toprule
        what & \textbf{85.49} & 80.57 & \textbf{77.22} & 70.84 \\ \hline
        who &  \textbf{88.73} & 83.31 & \textbf{81.01} & 74.05\\ \hline
        how & \textbf{78.89} & 74.05 & \textbf{62.22} & \textbf{62.22}\\ \hline
        why & \textbf{83.59} & 83.2 & \textbf{71.81} & 70\\ \hline
        assertion & \textbf{80.0}7 & 71.48 & 76.11 & \textbf{85.07}\\ \hline
        which & \textbf{74.13} & 70.69 & \textbf{74.13} & 70.69\\ \hline
        double questions &  \textbf{85.58} & 81.39 & \textbf{76.59} & 70.21\\ \hline
        when &  \textbf{83.33} & 82 & 72.09 & \textbf{74.41}\\ \hline
        where &  \textbf{85.91} & 78.17 & \textbf{75} & 72.22\\
    \bottomrule
    \end{tabular}
    \caption{Performance of QA and Neural models on heuristicaly determined question types in MultiRC}
    \label{tab:heuristic_categories_perf_multirc}
\end{table*}

\begin{table*}[!ht]
    \centering
    \begin{tabular}{p{0.6\textwidth}|l|p{0.2\textwidth}}
    \toprule
        \textbf{Example} & \textbf{Type} & \textbf{Remark}\\
    \toprule
        \textbf{Q:} What are two units of speed?
        & \multirow{2}{*}{what} & \multirow{2}{*}{Multiple answers}\\ 
        \textbf{A:} SI and MPH &&\\ \hline
        %
        \textbf{Q:} What was the names and locations of two peers of bin Ladin?
        & \multirow{2}{*}{what} & Multiple answers,\\
        \textbf{A:} Blind Sheik - New Jersey &&Partially correct \\ \hline
        %
        \textbf{Q:} What was Dennis Rodman's response when asked about his trip?
        & \multirow{2}{*}{what} & \multirow{2}{*}{Question in answer}\\
        \textbf{A:} When will we tire of this circus? &&\\ \hline
        %
        \textbf{Q:} Who are the characters in this story?
        & \multirow{2}{*}{who} & \multirow{2}{*}{Multiple answers}\\
        \textbf{A:} David and Alannah && \\ \hline
        %
        \textbf{Q:} Who are two members of Sarah's inner circle?
        & \multirow{2}{*}{who} & \multirow{2}{*}{Partially correct}\\ \textbf{A:} Ray &&\\ \hline
        %
        \textbf{Q:} Explain the religious schism in both England and Scotland.
        & \multirow{2}{*}{uncategorized} & \multirow{2}{*}{Hard for Conversion} \\
        \textbf{A:} Scotland was protestant &&\\ \hline
        %
        \textbf{Q:} What are the three ways in which Finnish reform can be seen?
        & \multirow{4}{*}{what} & Multiple answers, Partially correct\\
        \textbf{A:} The elevation of Finnish from a language of the common people to a national language equal to Swedish && \\
         
    \bottomrule
    \end{tabular}
    \caption{Example that are difficult for NLI under the constraints of the considered rules and neural model.}
    \label{tab:multirc_hard_examples}
\end{table*}

==> NLI for QA (StarSem Short Paper for Arxiv)/related_work2.tex <==
%% NLI Datasets and Models
\begin{figure*}
\centering
\begin{tabular}{cc}
  \includegraphics[width=0.4\linewidth, height=7cm]{images/for_conversion_qa_ex.png} \hspace{5mm}&   \includegraphics[width=0.4\linewidth, height=7cm]{images/for_conversion_nli_ex.png} \\
(a) QA sample & (b) Converted NLI sample \\[6pt]
\end{tabular}
\vspace{-4mm}
\caption{A RC sample with multiple answer choices converted to an NLI sample.}
\label{fig:conversion}
\end{figure*}

Reading comprehension (RC) is one of many potential downstream tasks that can benefit from NLI \cite{maccartney2009natural}. It is easy to see that RC naturally reduces to a two-class NLI problem; specifically, it can be cast as the task of identifying if a given piece of text entails the statement formed by converting a question and a potential answer to an assertive statement (hypothesis).

Given the intuitive conversion between RC and NLI, \citet{Demszky2018} designed both a rule-based conversion system as well as a trained neural model to convert question-answering datasets such as SQuAD \cite{rajpurkar2016squad} and RACE \cite{lai2017race} to an NLI form. However, it is unclear what these converted NLI datasets  offer compared to the original question-answering datasets w.r.t semantics. We show that converting a RC task to an NLI task helps in answering certain types of questions. This establishes the usefulness of the converted datasets. 

\citet{jin2019mmm} show that despite the different form of NLI and QA tasks, performing coarse pretraining of models on NLI datasets like SNLI \cite{Bowman2015} and MultiNLI \cite{mnli} not only improves the performance of these models on downstream reading comprehension tasks, but also helps with faster convergence. We show that -- for certain types of questions in reading comprehension datasets -- simply transforming the task to NLI can show improvement in performance, even without pretraining on any NLI dataset.

\citet{Trivedi2019} introduced a learnt weight-and-combine architecture to effectively re-purpose pretrained entailment models (trained on SNLI and MultiNLI) to solve the task of multi-hop reading comprehension. 
%They employ a learnt weight-and-combine approach to re-purpose NLI models trained on SNLI and MultiNLI to perform the task of RC.
%to combat the challenges posed by a long premise \kartik{Do you want to give them the long-premise credit? :) I wonder if there is a way to anonymously cite papers under submission} in question-answering tasks, and 
%They also perform several rule-based pre-processing steps on the RC dataset to convert it into the NLI form. 
They show that for certain datasets, this strategy can produce good results. 
%However, the models used in their study are not comparable with the current state-of-the-art QA models. 
However, their study focuses mainly on improving model performance using a pre-trained NLI model, and lacks an analysis of the reasoning differences arising due to the different form of the NLI and QA tasks. We focus our analysis on this aspect.


==> NLI for QA (StarSem Short Paper for Arxiv)/setup.tex <==


This section describes our experimental setup for comparing a QA based approach and an NLI based approach for the task of reading comprehension. We first obtain a parallel NLI and QA dataset by converting existing RC dataset into an NLI dataset. We then train two models, one on each form of the data, and analyse their performance.

==> artefacts.tex <==
%As a sanity check, we evaluated both the Rule-based NLI and QA models on an adversarial dev set consisting of examples from the original dev set replaced with static passages of the same length. This test was performed to reveal any artefacts in the data and/or conversion rules that might be resulting in the increase in performance. The results are mentioned in  Table \ref{tab:static-passage-results}. \todo{Fill in Missing Values in the table.}

%Both models gave similar performances, getting about $45\%$ accuracy. While the similar numbers confirm that the gain of the NLI model is not due to artefacts in the conversion rules, the high accuracy achieved by both models is indicative of caveats in the RACE dataset as well as the limitations of RoBERTa as a model.
We first present in Table \ref{tab:static-passage-results}, the performance of the trained models on the \emph{static-passage dev set} as these provide useful information regarding the model performance on the actual dev sets, discussed later.  
For the sake of brevity and easy reference, we call the classification model trained on the input formed by applying the rule-based conversion as the rule-based model.

% \subsection{Evaluation on static-passage dev sets}
For all the datasets in any format, we can see that the evaluation on the static-passage examples produces accuracies higher than random, implying that there are "easy" examples in the dev set which the models can solve without having any useful information in the passage/premise. 

While on RACE and RACE-subset, model trained on any format archives about 42-46\% accuracy on the corresponding static-passage dev set, we observe that on MultiRC the QA models consistently get better accuracy on the static-passage dev set. This indicates that when MultiRC is presented in the QA format, the model finds ways to answer the questions without looking at the passage. On the DREAM dataset, the model achieves about 38\% accuracy in both the QA and NLI formats. This is quite close to random performance, suggesting that the model does in fact use the passage to answer the questions.




%Contrary to the static passage evalutation on RACE-Subset, on the MultiRC dataset the QA version with question and answer concatenation leaks a larger percentage of the answers. As seen from Table \ref{tab:static-passage-results}, the QA model gets $62.2\%$ accuracy on the adversarial MultiRC dev set whereas the NLI model with neural conversions gets only $58.31\%$ which is fairly close to the majority class baseline. \comment{The models do not predict majority class which rules out a naive prediction criterion that the models might have used in the absence of a useful premise. Further, $55\%$ of the accuracy achieved by the QA model overlaps with it's predictions in the static passage setting whereas this overlap is only $44\%$ for the neural NLI model. Thus, the NLI model gains more ($35\%$) than the QA model ($30\%$) when the input contains a relevant premise.} We posit that the model is able to better exploit the artefacts in the dataset when the input is presented in a question-answer concatenation form as opposed to a well formed hypothesis\comment{, however, we are unable to characterize these artefacts}. We use these predictions to divide the dataset into \textit{Hard} and \textit{Easy} and analyse the performance of both the models on the \textit{Hard} questions which neither of the model is able to answer correctly in the static passage setting. The results are discussed in Section \ref{subsec:qualitative_heuristic_cat}.

%We also train the models without the passage/premise, giving only the answer options as input for the RACE-Subset dataset. Figures \ref{fig:random_seed_nli} and \ref{fig:random_seed_qa} show the learning curves of both the models over 3 epochs. Both models achieve close to $50\%$ accuracy with just the answer options further supporting the claim of existence of artefacts in the RACE dataset which the models are able to exploit.

%\begin{figure}[h]
 %   \centering
  %  \includegraphics[width=0.45\textwidth]{images/RandomSeed_NLI.png}
   % \caption{Training Rule-based NLI model without premise. The curves show 10 random seed runs.}
    %\label{fig:random_seed_nli}
%\end{figure}

%\begin{figure}[h]
 %   \centering
  %  \includegraphics[width=0.45\textwidth]{images/RandomSeed_QA.png}
   % \caption{Training QA model without passage. The curves show 10 random seed runs.}
    %\label{fig:random_seed_qa}
%\end{figure}

\begin{table*}[!ht]
\centering
\begin{tabular}{@{}lllllll@{}}
\toprule
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Random} & \multirow{2}{*}{Majority} & \multicolumn{4}{c}{Dataset Format (conversion method)}          \\ \cmidrule(l){4-7} 
                     &&& QA (None) & NLI (Rule-based) & NLI (Neural)      & NLI (Hybrid) \\ \toprule
RACE                    & 25.00 & 26.6 & 42.48& -& 43.01 & 42.95 \\
RACE-subset             & 25.00 & 27.2 & 45.50 & 45.90 & 44.23 & 45.20 \\\midrule
DREAM                   & 33.33 & 34.40 & 37.75 & -& 37.90&38.48\\
DREAM-subset            & 33.33 & 34.20 & 37.04 &37.77 & 38.38 & 38.08 \\\midrule
MultiRC                 & 50.00 & 57.19 & \textbf{62.21} & -& 58.31 & 57.34\\
MultiRC-subset          & 50.00 & 57.46& \textbf{64.19} & 59.6 & 57.80 & 58.00 \\
 \bottomrule
\end{tabular}
\caption{Accuracy numbers on the static-passage dev set with premise replaced with static text of equal length.}
\label{tab:static-passage-results}
\end{table*}


%% DO AGAIN
%Dream-subset QA, DREAM NLI(Neural), RACE-subset NLI(Neural), RACE-subset NLI (Hybrid), RACE NLI (hybrid), MultiRC NLI (hybrid)

==> contributions.tex <==
\section{Motivation}
\begin{itemize}
    \item 
    NLI is considered a fundamental task in natural language processing. However, application to downstream tasks such as QA is extremely limited with most QA task leaderboards being dominated by complex neural models trained specially for the downstream tasks. NLI-based knowledge transfer models fail miserably when compared to these models. The motivation of our work is to understand the usefulness of NLI and utilize it effectively for Question Answering.

    \item
    The ability to effectively convert downstream NLP tasks to textual entailment would allow the use of a common abstractive layer for training a model that understands the fundamentals of language and is able to transfer this knowledge across NLP tasks.
    
    \item
    State-of-the-art (BERT based) QA models seem to be approaching multiple choice question answering more like an NLI task rather than a QA task. i.e, each answer option is evaluated independently of the others. Restructuring the input and making it even more similar to NLI should boost performance.
\end{itemize}

\section{Contributions}
\begin{itemize}
    \item
    NLI is useful for QA.
    \begin{itemize}
        \item 
        \textit{Qualitative Analysis} of how NLI can be used to enhance QA performance: We present categories of questions which are better solved when posed as an entailment task than a QA task and vice versa.
        \item
        \textit{Quantitative Analysis} of how NLI can be used to enhance QA performance : We show concrete evidence that restructuring input as NLI improves near state-of-the art model performance.
        \item
        Benefits of pre-training and transfer learning ability of the NLI models. [Need to evaluate] 
    \end{itemize}
    
    \item
    BART-based dataset conversion.
    \begin{itemize}
        \item We provide a novel neural based model for effectively converting any QA dataset to NLI format while preserving grammatical structure.
        
        \item Evaluate the conversion on a QA downstream task [Need to evaluate]
        
        \item Better than rule-based conversion [Need to evaluate]
    \end{itemize}
\end{itemize}

\section{Related Work}
\begin{itemize}
    \item 
    No appreciable performance improvements over BERT-like models using NLI. Either prior work does not perform as well as SOTA or doesn't compare to SOTA. \cite{khot2018scitail, clark2018think, Clark, Clark2019, trivedi2019repurposing}

    \item
    Lack of qualitative analysis of NLI and QA tasks to understand model performance. \citet{richardson2019probing} analyse NLI but do not show how these categories might be related to performance on downstream tasks.
    
    \item
    Work done towards converting QA datasets to NLI have largely been rule based and have focused mainly on quality of conversion without attempting to evaluate the conversion on the downstream tasks. \cite{khot2018scitail, clark2018think, Demszky2018, trivedi2019repurposing}
    
    \item
    Pretraining on multiple NLI datasets to improve downstream task performance not done so far.
\end{itemize}


==> entailment_examples.tex <==
% \begin{table*}[!ht]
%     \centering
%     \begin{tabular}{p{3.5cm}|p{5.5cm}|p{5.5cm}}
%         \toprule
%         \textbf{Premise} & A senior is waiting at the window of a restaurant that serves sandwiches & \textbf{Relationship}\\
%         \bottomrule
%         \multirow{3}{*}{\textbf{Hypothesis}}& A person waits to be served his food & Entailment  \\
%         & A man is looking to order a grilled cheese sandwich & Neutral  \\
%     & A man is waiting in line for the bus & Contradiction \\
%         \bottomrule
%     \end{tabular}
%     \caption{Example of Natural Language Inference}
%     \label{tab:nli_example}
% \end{table*}

\begin{table*}[!ht]
    \centering
    \begin{tabular}{p{0.3\textwidth}|p{0.6\textwidth}}
        \toprule
        \textbf{Premise} & \textbf{Hypothesis}\\
        \bottomrule
        \begin{flushleft}
        A senior is waiting at the window of a restaurant that serves sandwiches\end{flushleft}
        & \begin{flushleft} (Entails)\break\textbf{Entailment:} A person waits to be served his food. \break
        
        (Not Entails)\break
        \textbf{Neutral:} A man is looking to order a grilled cheese sandwich. \break
        \textbf{Contradiction:} A man is waiting in line for the bus. \end{flushleft}\\
        \bottomrule
    \end{tabular}
    \caption{Example of Natural Language Inference}
    \label{tab:nli_example}
\end{table*}

==> experiments.tex <==
\subsection{Datasets}
\label{sec:datasets}
%\guide{Please list which datasets you plan to use , whether or not you have access them, and whether or not they are publicly available with the same preprocessing and train / dev / tests as the previous work you will be comparing to (if applicable).}
%\points{Write why we picked RACE. Problems with ARC/SciTail. What are the other datasets which we might use to establish/generalize our findings. How we are converting RACE dataset. }

While there are several QA datasets available, we will use RACE \cite{lai2017race}, MultiRC \cite{multirc} and OpenBookQA \cite{openbookqa} for our analysis, as these datasets provide variety in terms of the types of reasoning required to answer a question while also giving us an opportunity to compare our findings to other related work \cite{Trivedi2019}. 


The analysis in this work is focused on the task of multiple choice question answering. In order to compare the performance of the system using a QA model to that of the one using an NLI model, we will convert the QA datasets to NLI format where the question and answer option will be used to create a hypothesis sentence while the premise will consist of the passage/context text as shown in the figure \ref{fig:conversion_nli}. In order to perform the conversion, we will first employ rule based methods from \cite{Trivedi2019,Demszky2018} and move on to a neural conversion model proposed in \cite{Demszky2018} should we find the quality of rule based conversion unsatisfactory. 

 \begin{figure*}[!h]
    \centering
    \includegraphics[width=\linewidth]{images/conversion_pure_nli.png}
    \caption{Conversion of a QA sample into four NLI samples to be used in ``pure NLI'' setting.}
    \label{fig:conversion_nli}
\end{figure*} 

\subsection{Models}
%\guide{Please list the baseline methods (if applicable) that you will compare to, importantly state whether or not you will need to run their method on new datasets or if you have already published results. Also list if they have publicly available source code that can be used to run experiments.}



We divide our models into two general categories, namely large scale language model based (LSLM) and small entailment models (SEM). The LSLM category consists of RoBERTa \cite{liu2019roberta} and BERT \cite{devlin2018bert} sentence classification models consisting of the corresponding pretrained masked language model encoder at the base with sequence classification head. While SEM models consist of decomposable attention model (DecompAttn) \cite{parikh2016decomposable} and enhanced LSTM for NLI (ESIM) \cite{Chen} which are trained from scratch. Including these two categories of models in our analysis will help us quantify the effect of large scale pretraining with masked language modelling objective on the task of question answering through natural language inference.


\subsection{Training and Evaluation}
\label{sec:training}
We conduct experiments using two strategies. In one, which we call ``NLI with options'', we train and evaluate the model in a QA-like setting where each sample is treated as a 4-way classification problem as shown in the figure \ref{fig:conversion_nli_with_options} (right). The hypotheses for all of the answer options are fed to the network along with the premise (passage) to obtain a joint distribution over the hypothesis options. The only difference between this and a QA setting is that instead of feeding the model four question-option pairs we give the model four hypothesis statements from which it has to choose the most suitable one. This setting allows us to isolate the effect of presenting the options as well-formed hypothesis sentences instead of question+option sequence.

Alternatively, we also train and evaluate models in a much harder ``pure NLI'' setting where the hypothesis corresponding to each answer option is treated as an individual example during training. At evaluation time, we use the NLI scores - which are the scores obtained by passing each premise-hypothesis pair to the NLI model and select the correct answer as the option that gets the best score. This harder training objective forces the model to look for more evidence while selecting an answer hypothesis and is also suited for QA datasets like MultiRC where multiple options can be correct simultaneously.

\begin{figure*}[!h]
    \centering
    \includegraphics[width=\linewidth]{images/conversion_nli_with_options.png}
    \caption{Conversion of a QA sample into a single NLI sample to be used in the ``NLI with options'' setting.}
    \label{fig:conversion_nli_with_options}
\end{figure*} 
%\points{Two categories of models: LM based and non-LM based models. }

\subsection{Updates since the project proposal presentations}
%\points{Put the analysis from the dropbox paper}

We converted the RACE dataset into an entailment-based QA dataset as described in section \ref{sec:datasets}. We trained RoBERTa sequence classification model in both settings ``pure NLI'' as well as ``NLI with options'' and compared its performance to a RoBERTa QA model (trained on RACE dataset as it is). The accuracy on the dev dataset for all three settings is similar.
%shown in the table \ref{tab:roberta}. \lorraine{where is the table?}


%\begin{table*}[!ht]
%\centering
%\begin{tabular}{@{}llll@{}}
%\toprule
%Model   & \multicolumn{3}{c}{Accuracy on QA dev set} %              \\ \midrule
%        & Trained as QA & Trained as Pure NLI & Trained as NLI with options \\ \midrule
%RoBERTa-large &               &                     &                             \\ \bottomrule
%\end{tabular}
%\caption{Results for RoBERTa-large}
%\label{tab:roberta}
%\end{table*}


Even though the models perform similarly in all three settings, a deeper error analysis provides some interesting observations. While the RoBERTa QA model performs well on questions which can be answered using the surface information and which do not require multi-hop or complex reasoning, it fails to answer questions which require deeper understanding of the passage -- questions asking about a suitable title for the passage, or ones which ask about intentions of the author or people mentioned in the passage.


 
\subsection{Software}
We are using various set of open-source libraries for different subparts of this work. 
\begin{itemize}
    \item \textbf{Models}: While we are using HuggingFace's transformer\footnote{https://github.com/huggingface/transformers} library \cite{Wolf2019HuggingFacesTS} for pretrained language models like RoBERTa and BERT, we are using AI2's AllenNLP\footnote{https://github.com/allenai/allennlp/} \cite{Gardner2017AllenNLP} library to implement models like ESIM and DecompAttn. 
    
    \item \textbf{Analysis and Labeling}: We are using Label Studio \footnote{https://github.com/heartexlabs/label-studio} -- a multi-type data labeling and annotation tool -- for analysing, labelling and categorizing of our data.
    
    \item \textbf{Training management and hyperparameter tuning}: We are using Weights \& Biases\footnote{https://www.wandb.com/} \cite{wandb} to manage our experiments.
\end{itemize}



\subsection{Timeline}
%\guide{Please provide a week-by-week timeline for the next few weeks leading up to the midpoint presentations. What experiments will you do each week? What would you like to have accomplished by the midterm? If you're in a team how will you divide up the work?}

\begin{itemize}
    \item 03/08 - 03/14: 
    \begin{itemize}
        \item Implement ESIM and DecompAttn and train under all three settings mentioned in \ref{sec:training} (Dhruvesh)
        \item Implement other models in the LSLM category and train under all three settings (Anshuman)
        \item Categorize the erroneous as well correct predictions from RoBERTa sequence classification model on RACE as ``pure NLI'' and ``NLI with options'' and compare it with the errors made by the RoBERTa QA model on the RACE dataset (Aparna)
    \end{itemize}
    \item 03/15 - 03/21:
    \begin{itemize}
        \item Evaluate all the models on MultiRC and OpenBookQA in all three training settings (Dhruvesh, Anshuman, Aparna)
    \end{itemize}
    \item 03/21 - 03/27:
    \begin{itemize}
        \item Perform error analysis for all the models on all the datasets. Come up with general observations based on model category and dataset (Dhruvesh, Anshuman, Aparna)
        \item Work on mid-point presentation (Dhruvesh, Anshuman, Aparna)
    \end{itemize}
\end{itemize}

\subsection{Challenges}
%\guide{Lay down the challenges that you can foresee which might prevent you from attaining your goal.}

We are already facing several challenges and following are the major ones.

\begin{enumerate}
    \item \textbf{Grammaticality of hypothesis}: Due to the richness and variety of the questions, rule based methods to convert a question+answer option to a hypothesis sentence, in some cases, produce grammatically incorrect sentences. Currently, for the converted RACE dataset, we have identified that about 20\% of the total hypothesis sentences are grammatically incorrect. As this is a significant fraction, we continue to improve the employed rules to convert all such examples correctly. Since this aspect is not the  focus of this work, we do not wish to spend a lot of time on improving the conversion strategy.
    
    %\lorraine{how much percent of the converted sentence is un-grammatical? If not too much, we don't have to worry about this. But if it's a lot, maybe we should see the performance difference if we manually change some of the sentence into grammatically correct one?}
    
    \item \textbf{Long premise length}: Since the passage/context directly acts as the premise, on an average, we deal with premise sequences of 300 or more tokens. This poses two challenges. One, we cannot directly employ some of the BiLSTM based NLI models like ESIM as they cannot handle such long premise directly. Secondly, we cannot transfer learn from existing NLI datasets. We address the first issue by using Multee \cite{Trivedi2019} which employs small entailment models like ESIM with importance weighting and aggregation. 
\end{enumerate}


%\subsection{Contingency Plan}


==> further_exp.tex <==
\begin{itemize}
    \item
    Evaluate model performance with neural converted dataset.
    
    \item 
    Evaluate other datasets
    \begin{itemize}
        \item \textit{DREAM} - a multiple-choice Dialogue-based REAding comprehension exaMination dataset. \cite{sun2019dream} 
        
        It contains 10,197 multiple choice questions for 6,444 dialogues, collected from English-as-a-foreign-language examinations designed by human experts. 
        
        The dataset is likely to present significant challenges for existing reading comprehension systems: 84\% of answers are non-extractive, 85\% of questions require reasoning beyond a single sentence, and 34\% of questions also involve commonsense knowledge. 
        
        \item \textit{MultiRC} - a dataset of short paragraphs and multi-sentence questions that can be answered from the content of the paragraph. \cite{MultiRC2018}
        
        The entire corpus consists of ~10K questionss (~6k multiple-sentence questions). We release about 60\% of this data as training/dev data.
 
    \end{itemize}
    
    \item 
    Refine categories and perform more annotation.
    
    \item 
    Pre-train on other NLI datasets and evaluate performance.
\end{itemize}

==> reasoning_categories.tex <==
In order to get a qualitative understanding of the differences between the two settings, we divide the questions into $7$ categories reflecting the type of reasoning required to answer the question. Table \ref{tab:reasoning_categories} describes these reasoning categories along with examples.

\begin{table*}[!ht]
    \centering
    \begin{tabular}{p{3.5cm}|p{5.5cm}|p{5.5cm}}
        \toprule
        \textbf{Category} & \textbf{Description} & \textbf{Example}\\
        \bottomrule
        Linguistic Matching & Can be answered merely by matching words between the question and a sentence from the passage & \textbf{Passage Sentence:} Food cooks quickly in parabolic cookers \\ & & \textbf{Question:}If you want to cook food quickly, which kind of sun-cooker is your best choice?\\\hline
        Main Idea & Require topicality judgements & What's the best title for this passage?\\\hline
        Negation & Picking the wrong/incorrect statement & Which of the following statements is NOT true?\\\hline
        Dialogue & Can be inferred from a dialogue or direct speech in the passage & By saying "her pen dared travel where her eyes would not", the writer means\\\hline
        Math & Counting or mathematically combining facts & How many functions of snow are discussed in the passage?\\\hline
        Deductive & None of the above but can be answered precisely from the premise text & Which of the following statements is TRUE?\\\hline
        Inductive & None of the above and cannot be answered precisely from the text & How old is most likely the writer's father?\\
        \bottomrule
    \end{tabular}
    \caption{Reasoning Categories}
    \label{tab:reasoning_categories}
\end{table*}

We construct the delta region as the $328$ dev set examples on which the predictions of the QA and Rule-based NLI models differ. We further divide the Delta region into Gain (NLI gets it right, QA gets it wrong) and Loss (QA gets it right, NLI gets it wrong). We annotate these $328$ ($192$ in Gain and $136$ in Loss) examples into one of the $7$ categories. The annotation process also revealed that about half the examples were not properly converted by the rules leading to grammatical errors or loss of information in conversion. For the purpose of our analysis, we removed these examples leaving a total of $175$ examples ($109$ in Gain and $66$ in Loss). However, it's worth noting that the presence of bad conversions affects the scope of learning of the model in addition to the fact the fraction of incorrect conversions was higher in the Loss region. These observations suggest that improving upon conversion could further boost performance.

Figure \ref{fig:gain_dist} and \ref{fig:loss_dist} show the distribution of labels over the Gain and Loss regions respectively. The distribution reflects that the QA models clearly outperforms the NLI model in negation questions whereas the NLI model outperforms the QA model in dialogue and deductive reasoning categories.

\begin{figure}[h]
\includegraphics[width=0.45\textwidth]{images/Gain_QAvsRule.png}
\caption{Distribution of Reasoning Categories over the Gain region - Rule-based NLI vs QA model}
\label{fig:gain_dist}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{images/Loss_QAvsRule.png}
    \caption{Distribution of Reasoning Categories over the Loss region - Rule-based NLI vs QA model.}
    \label{fig:loss_dist}
\end{figure}

==> reasoning_categories_heuristical.tex <==
\begin{table*}[!ht]
    \centering
    \begin{tabular}{p{0.25\textwidth}|p{0.65\textwidth}}
        \toprule
        \textbf{Type} & \textbf{Heuristics} \\
        \bottomrule
        Main Idea & Questions containing the words 'mainly', 'title', 'purpose' or 'topic'\\\hline
        Negation & Questions containing the 'not', 'except' or 'which of the following is wrong'\\\hline
        Dialogue & Passages containing more than 10 quotation marks (")\\\hline
        Math & Questions containing the words 'how many', 'how old' or 'how much'\\\hline
        Deductive & Questions containing the word 'true'\\\hline
        Fill in the Blanks (FITB) & Questions containing a blank (\_)\\
        \bottomrule
    \end{tabular}
    \caption{Heuristically Determined Question Types - RACE}
    \label{tab:heuristic_categories}
\end{table*}

As a consequence of the rule-based conversion strategy, we unintentionally get 2 very different sets of data from the RACE dataset. $83\%$ of the RACE-subset consists of questions with question-words such as \{\textit{who, what, when, where, why, which, how}\} whereas only $1\%$ of the rest of the RACE dataset has such questions. Conversely, only about $11\%$ of the subset consists of fill-in-the-blanks (FITB) questions whereas $95\%$ of the rest of the dataset has FITB questions. \comment{FITB questions are largely with the blank towards the end of the question and a question-answer concatenation strategy turns out to be very similar to a coherent conversion strategy. We argue that this is the reason for equivalent performance of the models on the FITB part of the data. However, on the RACE-subset, NLI models are able to outperform the QA model which showing the clear benefits of coherent conversion on complex question formulations.}

In order to compare the models trained using the neural and hybrid conversion to the rule-based conversion, we define some non-exclusive categories using heuristics, as described in Table \ref{tab:heuristic_categories}. We observe that the NLI model which uses the hybrid conversion gets a significantly better performance on the deductive reasoning category than the NLI model which uses the rule-based conversion. This observation is consistent with the trend seen in the comparison of the rule-based model vs the QA model, where the rule-based model outperforms the QA model on the deductive reasoning category. Additionally, the rule-based model outperforms the QA model significantly in the dialogue category. Table \ref{tab:heuristic_categories_perf} shows the performance of the models on the RACE-subset dataset over these question types. This trend further emphasizes the benefits of proper hypothesis generation as opposed to question and answer concatenation for the question-answering task.

On the Multi-RC dataset, we created question types by following heuristics similar to those used in the orignal paper to analyse the dataset distribution. The question types and their proportion in the dataset is described in Table \ref{tab:heuritic_categories_multirc}. We analyse the performance of both the QA and neural-conversion NLI model across these categories. Specifically, we analyse the changes in trend on the subset of \textit{Hard} questions (Section \ref{subsec:qualitative_artefacts}). The distribution across categories does not change in the restricted set of \textit{Hard} questions which indicates that the artefacts are not specific to any of these question types. We observe that the NLI model outperforms the QA model on \textit{assertion} and \textit{when} types and matches QA performance on \textit{how} questions. To further understand the performance gap, we looked examples from these different categories and found that there are certain complexities in the questions which neural conversion is unable to handle. These include questions with multiple answers, examples where the answer is also a question and examples with partially correct answers labelled as true in the dataset. Table \ref{tab:multirc_hard_examples} provides some examples of these. Such examples are also a major cause for incorrect conversions. It is particularly interesting to note that such difficult examples are present in \textit{what} and \textit{who} in large proportions and almost completely absent from question types such as \textit{assertion}. This could be the primary reason for the inability of the NLI model to beat or even match QA model performance on these categories. We conclude that MultiRC is a harder dataset for NLI in the constraints of the rules and neural model we have trained. The dataset has nuances which need to be captured during conversion to be able to outperform the QA model.

\begin{table}[!ht]
    \centering
    \begin{tabular}{c|c|c|c}
        \toprule
        \textbf{Type} & \textbf{QA} & \textbf{Rule-based} & \textbf{Hybrid}\\
        \bottomrule
        Main Idea & 84.19 & \textbf{84.83} & \textbf{84.83}\\\hline
        Negation & \textbf{80.86} & 77.77 & 79.01\\\hline
        Dialogue & 80.65 & \textbf{83.60} & 82.95\\\hline
        Math & 45 & \textbf{55} & \textbf{55}\\\hline
        Deductive & 81.91 & \textbf{88.29} & \textbf{90.42}\\\hline
        FITB & 79.02 & 79.02 & \textbf{79.40}\\
        \bottomrule
    \end{tabular}
    \caption{Model performances on heuristically determined question types for RACE-Subset}
    \label{tab:heuristic_categories_perf}
\end{table}


\begin{table*}[!ht]
    \centering
    \begin{tabular}{@{}l|p{0.35\textwidth}|p{0.35\textwidth}@{}}
    \toprule
        \textbf{Type} & \textbf{Heuristic} & \textbf{Example}\\
    \toprule
        what (40\%) 
 & Starts With ['What', 'In what', 'With what', 'To what'] or Ends With [‘what?’]
 & What is the drawback of kinetic energy from hydro power? \\ \hline
        who (15\%) & Starts With ['Who', 'Whom', 'With whom', 'From whom', 'For whom'] or Ends With [‘who?’, ‘whom?’] & Who does Billy have the same color hair as?\\ \hline
        how (12\%)& Starts With [‘How’] & Approximately how much older is Charlie than Sylvia?\\ \hline
        why (10\%)& Starts With [‘Why’] & Why did Phoebe cry?\\ \hline
        assertion (5\%)& Starts With ['Could it', 'Will ', 'Was', 'Were', 'Has', 'Have', 'Does', 'Would', 'Did', 'Had', 'Is', 'Are', 'Do', 'Can', 'True or false'] & Was the Emperor hurt when the explosion damaged his carriage?\\ \hline
        which (5\%) & Starts With ['Which', 'In which'] & Which philosopher is said to have taught the young Confucius?\\ \hline
        double questions (4.5\%) & Contains ['and what', 'and how', 'and which', 'and where', 'and when', 'and why', 'and by whom', 'if not, what?'] or count("?") $>$ 1 & Where did money to fund the 9/11 plotters come from and where didn't it come from?\\ \hline
        when (3\%) & Starts With [‘When’]
 & When did the Romans set up a fortress at Aquae Sextiae (Aix-en-Provence)?\\ \hline
        where (3\%) & Starts With [‘Where’] or Ends With [‘where?’]
 & Where does the absorption part of digestion occur?\\
    \bottomrule
    \end{tabular}
    \caption{Heuristicaly Determined Question Types - MultiRC}
    \label{tab:heuritic_categories_multirc}
\end{table*}

\begin{table*}[!ht]
    \centering
    \begin{tabular}{@{}lcccc@{}}
    \toprule
        \multirow{2}{*}{\textbf{Type}} 
            & \multicolumn{2}{c}{\textbf{All Questions}} & \multicolumn{2}{c}{\textbf{Hard Questions}}\\
            \cmidrule(l){2-3} \cmidrule(l){4-5} 
            & \textbf{QA} & \textbf{NLI (Neural)} & \textbf{QA} & \textbf{NLI (Neural)} \\
    \toprule
        what & \textbf{85.49} & 80.57 & \textbf{77.22} & 70.84 \\ \hline
        who &  \textbf{88.73} & 83.31 & \textbf{81.01} & 74.05\\ \hline
        how & \textbf{78.89} & 74.05 & \textbf{62.22} & \textbf{62.22}\\ \hline
        why & \textbf{83.59} & 83.2 & \textbf{71.81} & 70\\ \hline
        assertion & \textbf{80.0}7 & 71.48 & 76.11 & \textbf{85.07}\\ \hline
        which & \textbf{74.13} & 70.69 & \textbf{74.13} & 70.69\\ \hline
        double questions &  \textbf{85.58} & 81.39 & \textbf{76.59} & 70.21\\ \hline
        when &  \textbf{83.33} & 82 & 72.09 & \textbf{74.41}\\ \hline
        where &  \textbf{85.91} & 78.17 & \textbf{75} & 72.22\\
    \bottomrule
    \end{tabular}
    \caption{Performance of QA and Neural models on heuristicaly determined question types in MultiRC}
    \label{tab:heuristic_categories_perf_multirc}
\end{table*}

\begin{table*}[!ht]
    \centering
    \begin{tabular}{p{0.6\textwidth}|l|p{0.2\textwidth}}
    \toprule
        \textbf{Example} & \textbf{Type} & \textbf{Remark}\\
    \toprule
        \textbf{Q:} What are two units of speed?
        & \multirow{2}{*}{what} & \multirow{2}{*}{Multiple answers}\\ 
        \textbf{A:} SI and MPH &&\\ \hline
        %
        \textbf{Q:} What was the names and locations of two peers of bin Ladin?
        & \multirow{2}{*}{what} & Multiple answers,\\
        \textbf{A:} Blind Sheik - New Jersey &&Partially correct \\ \hline
        %
        \textbf{Q:} What was Dennis Rodman's response when asked about his trip?
        & \multirow{2}{*}{what} & \multirow{2}{*}{Question in answer}\\
        \textbf{A:} When will we tire of this circus? &&\\ \hline
        %
        \textbf{Q:} Who are the characters in this story?
        & \multirow{2}{*}{who} & \multirow{2}{*}{Multiple answers}\\
        \textbf{A:} David and Alannah && \\ \hline
        %
        \textbf{Q:} Who are two members of Sarah's inner circle?
        & \multirow{2}{*}{who} & \multirow{2}{*}{Partially correct}\\ \textbf{A:} Ray &&\\ \hline
        %
        \textbf{Q:} Explain the religious schism in both England and Scotland.
        & \multirow{2}{*}{uncategorized} & \multirow{2}{*}{Hard for Conversion} \\
        \textbf{A:} Scotland was protestant &&\\ \hline
        %
        \textbf{Q:} What are the three ways in which Finnish reform can be seen?
        & \multirow{4}{*}{what} & Multiple answers, Partially correct\\
        \textbf{A:} The elevation of Finnish from a language of the common people to a national language equal to Swedish && \\
         
    \bottomrule
    \end{tabular}
    \caption{Example that are difficult for NLI under the constraints of the considered rules and neural model.}
    \label{tab:multirc_hard_examples}
\end{table*}
